R2H: Building Multimodal Navigation Helpers that Respond to Help Requests

Intelligent navigation-helper agents are critical as they can navigate users in unknown areas through environmental awareness and conversational ability, serving as potential accessibility tools for individuals with disabilities. In this work, we first introduce a novel benchmark, Respond to Help Requests (R2H), to promote the development of multi-modal navigation helpers capable of responding to requests for help, utilizing existing dialog-based embodied datasets. R2H mainly includes two tasks: (1) Respond to Dialog History (RDH), which assesses the helper agent's ability to generate informative responses based on a given dialog history, and (2) Respond during Interaction (RdI), which evaluates the effectiveness and efficiency of the response during consistent cooperation with a task performer. Furthermore, we explore two approaches to construct the navigation-helper agent, including fine-tuning a novel task-oriented multi-modal response generation model that can see and respond, named SeeRee, and employing a multi-modal large language model in a zero-shot manner. Analysis of the task and method was conducted based on both automatic benchmarking and human evaluations. Project website: https://sites.google.com/view/response2helprequests/home.

==> table/Table_00_full.tex <==

\begin{table*}[t]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llll}
    \toprule
          \multicolumn{4}{m{20cm}}{
          $\begin{array}{rl}
              \textbf{Prompt:} & \text{Commander says: `Yes to the kitchen. Go to the left of the fireplace and then all the way up the stairs'. } \\
              & \text{Step by step: 1. Yes. 2. go to the kitchen 3. go the left of the fireplace, 4. go upstairs.}\\
              & \text{Commander says:\_\_\_\_. step by step: 1.}
          \end{array}$
       }\\
          \toprule
          \textbf{Index}&\multicolumn{1}{c}{\textbf{Original response}} & \multicolumn{2}{c}{\textbf{Processed response}} \\
          \toprule
          1 &\multicolumn{1}{l}{Go into the bedroom and walk through it and exit it by using a door on the left.} & \multicolumn{2}{l}{$\begin{array}{l}
               \text{1. Enter the bedroom. }\\
                \text{2. Walk through it.}\\ 
                \text{3. Exit by using a door on the left.}
          \end{array}$} \\
          \cmidrule(lr){2-4} 
          2 &\multicolumn{1}{l}{Yeah keep going around the outside till you get to the end. And sorry about the mixup at first.} & \multicolumn{2}{l}{$\begin{array}{l}
               \text{1. Yeah.}\\
                \text{2. Keep going around the outside.}\\ 
                \text{3. Get to the end.}
          \end{array}$} \\
          \cmidrule(lr){2-4} 
          3 &\multicolumn{1}{l}{Go straight a little, then the right and go downstairs.} & \multicolumn{2}{l}{$\begin{array}{l}
               \text{1. Go straight a little.}\\
                \text{2. Go right.}\\ 
                \text{3. Go downstairs.}
          \end{array}$} \\
          \cmidrule(lr){2-4} 
          4 &\multicolumn{1}{l}{I would go back.} & \multicolumn{2}{l}{$\begin{array}{l}
               \text{1. Go back.}
          \end{array}$} \\
         \bottomrule
    \end{tabular}}
    \caption{Examples of our Parse by Step method on the CVDN dataset~\cite{thomason2020vision}. We fill the original response to the blank of the prompt and input to GPT-3 for sentence completion. The output from the GPT-3 becomes the processed response with mainly task-related instructions kept and organized in steps. Through Parse by Step, we preprocess the response in the training set.}
    \label{tab:table_00}
\end{table*}

==> table/Table_22.tex <==
% \usepackage{tabularray}


==> table/Table_3.tex <==


\begin{table}[t]
    \centering
\setlength{\abovecaptionskip}{0.1cm}
\setlength\tabcolsep{-1pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llc|ccc|ccc} 
\toprule
% && \multicolumn{8}{|c|}{\textbf { Seen Validation }} & \multicolumn{8}{|c|}{\textbf { Unseen Validation }}& \multicolumn{8}{c}{\textbf { Unseen Testing }} \\
% \hline \multicolumn{1}{r}{\textbf{Task}} 
\multicolumn{3}{c|}{}& \multicolumn{3}{c|}{$\begin{array}{c}
     \textbf{Seen}  \\
     \textbf{Validation}
\end{array}$} & \multicolumn{3}{c}{$\begin{array}{c}
     \textbf{Unseen}  \\
     \textbf{Validation}
\end{array}$}\\
 \cmidrule(lr){4-6} 
 \cmidrule(lr){7-9} 

\multicolumn{2}{c|}{\textbf{Helper}} &
\multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}\\
     \textbf{Performer}
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$}
& \multicolumn{1}{r|}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$}& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$}\\



\midrule
%  & \text{Rule-based}  & 4.0  & 4.1   &  5.3   & 0.80  & 0.0  & 0.0  & 0.80   & 0.80  & 5.6 & 5.8 & 1.6 & 0.80 & 0.5 &0.5 & 5.1 & 0.81 & 3.4 & 3.6 & 3.3 & 0.80 & 0.0 & 0.0 & 3.3 & 0.82 \\
% \cmidrule(lr){0-1}
\multicolumn{2}{l|}{$\begin{array}{l}
    \text{RMM }\mathcal{G}\\
\end{array}$} & \multirow{3}{*}{$\begin{array}{l}
    \text{RMM}\\
    \mathcal{N}+\mathcal{Q}\\
\end{array}$}  & 1.39 & 3.33 & 10.67 & 0.82 & 1.18 & 4.86  \\

%  \multicolumn{3}{l|}{$\begin{array}{l}
%     \text{Fixed all speakers}\\
% \end{array}$}   & 1.52 & 5.55 & 10.49 & 0.54 & 1.57 & 5.38  \\
 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{RMM }\mathcal{G}\text{ (Fixed)}
\end{array}$} &  & 1.70 & 3.33 & 9.55 & 0.66 & \textbf{2.36} & 5.41  \\
 \multicolumn{2}{l|}{$\begin{array}{l}
    \text{SeeRee (ours)}\\
\end{array}$} &   & \textbf{2.33} & \textbf{5.55} & \textbf{10.74} & \textbf{0.87} & 1.57 & \textbf{5.55}  \\
% \midrule
% $\begin{array}{r}
%     \text {Human}\\
% \end{array}$   & \multicolumn{2}{c}{5.13}  & \multicolumn{2}{c}{5.13} & \multicolumn{2}{c}{0.49} & \multicolumn{2}{c}{0.33}   \\

\bottomrule
\end{tabular}
}
\caption{Results of evaluating different helper agents with the performer agent formed by the RMM Navigator model ($\mathcal{N}$) and RMM Questioner model ($\mathcal{Q}$) \cite{roman2020rmm} on the two-agent task built on CVDN \cite{thomason2020vision}. Our SeeRee agent enables the best two-agent training results.  
%\xin{there is no ``fixed'' results for SeeRee.}
\label{tab:table_3} }
% \vspace{-3mm}
\end{table}




==> table/copy.tex <==

\begin{table*}[t]
\setlength{\abovecaptionskip}{0.1cm}
    \centering

\begin{subtable}[t]{0.48\textwidth}
\resizebox{\columnwidth}{!}{
\setlength\tabcolsep{0pt}
\begin{tabular}{llc|ccc|ccc|cc|cc|ccc|ccc} 
\toprule
% && \multicolumn{8}{|c|}{\textbf { Seen Validation }} & \multicolumn{8}{|c|}{\textbf { Unseen Validation }}& \multicolumn{8}{c}{\textbf { Unseen Testing }} \\
% \hline \multicolumn{1}{r}{\textbf{Task}} 
\multicolumn{3}{c|}{}& \multicolumn{3}{c|}{$\begin{array}{c}
     \textbf{Seen}  \\
     \textbf{Validation}
\end{array}$} & \multicolumn{3}{c}{$\begin{array}{c}
     \textbf{Unseen}  \\
     \textbf{Validation}
\end{array}$}\\
 \cmidrule(lr){4-6} 
 \cmidrule(lr){7-9} 

\multicolumn{2}{c|}{\textbf{Helper}} &
\multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}\\
     \textbf{Performer}
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$}
& \multicolumn{1}{r|}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$}& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$}\\
\midrule
%  & \text{Rule-based}  & 4.0  & 4.1   &  5.3   & 0.80  & 0.0  & 0.0  & 0.80   & 0.80  & 5.6 & 5.8 & 1.6 & 0.80 & 0.5 &0.5 & 5.1 & 0.81 & 3.4 & 3.6 & 3.3 & 0.80 & 0.0 & 0.0 & 3.3 & 0.82 \\
% \cmidrule(lr){0-1}
\multicolumn{2}{l|}{$\begin{array}{l}
    \text{Human Annotator}\\
\end{array}$} & \multirow{4}{*}{$\begin{array}{l}
    \text{HAMT}
\end{array}$}  & 6.9 & 17.6 & 20.7 & 5.1 & 11.2 & 17.1  \\
\cmidrule(lr){0-1}
\cmidrule(lr){4-9}

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{RMM }\mathcal{G}
\end{array}$} &  & 4.7 & 8.6 & 14.4 & 2.8 & 6.8 & 10.7  \\

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{Multimodal LLM}
\end{array}$} &  & 5.3 & \textbf{14.7} & 17.5 & 3.6 & 8.2 & 13.1  \\

 \multicolumn{2}{l|}{$\begin{array}{l}
    \text{SeeRee}\\
\end{array}$} &   & \textbf{6.5} & 14.0 & \textbf{17.8} & \textbf{4.9} & \textbf{10.1} & \textbf{15.2}  \\

\bottomrule
\end{tabular}
}
\caption{CVDN dataset}
\end{subtable}

\begin{subtable}[t]{0.48\textwidth}
\setlength\tabcolsep{2pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llc|cc|cc} 
\toprule

\multicolumn{3}{c|}{}& \multicolumn{2}{c|}{$\begin{array}{c}
     \textbf{Seen}  \\
     \textbf{Validation}
\end{array}$} & \multicolumn{2}{c}{$\begin{array}{c}
     \textbf{Unseen}  \\
     \textbf{Validation}
\end{array}$}\\
 \cmidrule(lr){4-5} 
 \cmidrule(lr){6-7} 

\multicolumn{2}{c|}{\textbf{Helper}} &
\multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}\\
     \textbf{Performer}
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$}
& \multicolumn{1}{r|}{$\begin{array}{r}
     \text{PWSR}\uparrow
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{PWSR}\uparrow
\end{array}$}\\
\midrule

\multicolumn{2}{l|}{$\begin{array}{l}
    \text{Human Annotator}\\
\end{array}$} & \multirow{4}{*}{$\begin{array}{l}
    \text{DialFRED}\\
    \text{Performer}
\end{array}$}  & 49.1 & 39.1 & 33.4 & 14.6  \\
\cmidrule(lr){0-1}
\cmidrule(lr){4-7}

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{RMM }\mathcal{G}
\end{array}$} &  & 46.5 & 35.3 & 32.1 & 13.8  \\
\multicolumn{2}{l|}{$\begin{array}{c}
    \text{Multimodal LLM}
\end{array}$} &  & 47.0  & 32.5 & \textbf{33.8}  & 14.2 \\
 \multicolumn{2}{l|}{$\begin{array}{l}
    \text{SeeRee}\\
\end{array}$} &   & \textbf{49.1} & \textbf{39.1} & 33.1 & \textbf{14.3}  \\

\bottomrule
\end{tabular}
}
\caption{DialFRED dataset}
\end{subtable}


\begin{subtable}[t]{0.48\textwidth}
\resizebox{\columnwidth}{!}{
\setlength\tabcolsep{0pt}
\begin{tabular}{llc|ccc|ccc} 
\toprule

\multicolumn{3}{c|}{}& \multicolumn{3}{c|}{$\begin{array}{c}
     \textbf{Seen}  \\
     \textbf{Validation}
\end{array}$} & \multicolumn{3}{c}{$\begin{array}{c}
     \textbf{Unseen}  \\
     \textbf{Validation}
\end{array}$}\\
 \cmidrule(lr){4-6} 
 \cmidrule(lr){7-9} 

\multicolumn{2}{c|}{\textbf{Helper}} &
\multicolumn{1}{c|}{$\begin{array}{c}
     \textbf{Task}\\
     \textbf{Performer}
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$}
& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$}
& \multicolumn{1}{r|}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{GP}\uparrow
\end{array}$}& \multicolumn{1}{r}{$\begin{array}{r}
     \text{SPL}\uparrow
\end{array}$} & \multicolumn{1}{r}{$\begin{array}{r}
     \text{SR}\uparrow
\end{array}$}\\
\midrule
\multicolumn{2}{l|}{$\begin{array}{l}
    \text{Human Annotator}\\
\end{array}$} & \multirow{4}{*}{$\begin{array}{c}
    \text{HAA-}\\
    \text{Transformer}
\end{array}$}  & 56.3 & 14.7 & 17.3 & 55.2 & 16.5 & 20.4  \\
\cmidrule(lr){0-1}
\cmidrule(lr){4-9}

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{RMM }\mathcal{G}
\end{array}$} &  & -37.0 & 2.4 & 3.5 & -26.6 & 3.6 & 4.9  \\

 \multicolumn{2}{l|}{$\begin{array}{c}
    \text{Multimodal LLM}
\end{array}$} &  & -96.5 & 0.7 & 0.8 & -95.9 & 1.5 & 2.2  \\

 \multicolumn{2}{l|}{$\begin{array}{l}
    \text{SeeRee}\\
\end{array}$} &   & \textbf{-29.6} & \textbf{4.6} & \textbf{5.7} & \textbf{-24.9} & \textbf{4.4} & \textbf{6.1}  \\

\bottomrule
\end{tabular}
}
\caption{AVDN dataset}
\end{subtable}





\caption{Results of Respond to Dialog History (RDH) task on CVDN dataset (a) and DialFRED dataset (b) \cite{thomason2020vision,gao2022dialfred}. We replace the response in validation sets with responses from different helper agents. Since the task performer agent is trained with human dialog and is fixed, it relies on the information contained in the response to complete the task. Thus, the better the task performer agent performs in the task, the more effective the response is.\jing{test}}
\label{tab:table_0_1}
\end{table*}

